One for All: Towards Training One Graph Model for All Classification Tasks

Designing a single model to address multiple tasks has been a long-standing objective in artificial intelligence. Recently, large language models have demonstrated exceptional capability in solving different tasks within the language domain. However, a unified model for various graph tasks remains underexplored, primarily due to the challenges unique to the graph learning domain. First, graph data from different areas carry distinct attributes and follow different distributions. Such discrepancy makes it hard to represent graphs in a single representation space. Second, tasks on graphs diversify into node, link, and graph tasks, requiring distinct embedding strategies. Finally, an appropriate graph prompting paradigm for in-context learning is unclear. We propose \textbf{One for All (OFA)}, the first general framework that can use a single graph model to address the above challenges. Specifically, OFA proposes text-attributed graphs to unify different graph data by describing nodes and edges with natural language and uses language models to encode the diverse and possibly cross-domain text attributes to feature vectors in the same embedding space. Furthermore, OFA introduces the concept of nodes-of-interest to standardize different tasks with a single task representation. For in-context learning on graphs, OFA introduces a novel graph prompting paradigm that appends prompting substructures to the input graph, which enables it to address varied tasks without fine-tuning. We train the OFA model using graph data from multiple domains (including citation networks, molecular graphs, knowledge graphs, etc.) simultaneously and evaluate its ability in supervised, few-shot, and zero-shot learning scenarios. OFA performs well across different tasks, making it the first general-purpose across-domains classification model on graphs.

==> tables/zero_shot.tex <==
\begin{table}[t]
\centering
\small
\caption{Few-shot results (Acc) on cora, ogbn-arxiv, and ogbg-molpcba}
\setlength{\tabcolsep}{4.4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lllllll}
\toprule
Dataset     & \multicolumn{2}{c}{Cora}    & \multicolumn{2}{c}{ogbn-arxiv} & \multicolumn{2}{c}{ogbg-molpcba} \\
Type        & \multicolumn{2}{c}{Node} & \multicolumn{2}{c}{Node} & \multicolumn{2}{c}{Graph}   \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}

Task        & 2-way & 5-way  & 2-way   & 5-way  & 2-way  & 5-way  \\
\midrule
\midrule
Baseline               &   &    &     &    &     &    \\

\midrule

OFA &   &   &     &    &  &  \\
\bottomrule

\end{tabular}
\label{tabmain}
\end{table}


==> tex/6_limitations.tex <==
\section{Limitations and future works}
While OFA aims to provide a solution for the general graph foundation model, it is not yet able to perform regression tasks, which is an important direction we aim to research further. OFA is already trained in several different domains, and the performance is on par or even outperforms some GNN and LLM approaches. However, the training data for the graph foundation model is still scarce compared to that of LLMs. In the future, we plan to enhance model by contrastive learning and incorporate more data to improve the model generality.
